Contrastive Pre-Training with Multi-View Fusion for No-Reference Point Cloud Quality Assessment

No-reference point cloud quality assessment (NR-PCQA) aims to automatically evaluate the perceptual quality of distorted point clouds without available reference, which have achieved tremendous improvements due to the utilization of deep neural networks. However, learning-based NR-PCQA methods suffer from the scarcity of labeled data and usually perform suboptimally in terms of generalization. To solve the problem, we propose a novel contrastive pre-training framework tailored for PCQA (CoPA), which enables the pre-trained model to learn quality-aware representations from unlabeled data. To obtain anchors in the representation space, we project point clouds with different distortions into images and randomly mix their local patches to form mixed images with multiple distortions. Utilizing the generated anchors, we constrain the pre-training process via a quality-aware contrastive loss following the philosophy that perceptual quality is closely related to both content and distortion. Furthermore, in the model fine-tuning stage, we propose a semantic-guided multi-view fusion module to effectively integrate the features of projected images from multiple perspectives. Extensive experiments show that our method outperforms the state-of-the-art PCQA methods on popular benchmarks. Further investigations demonstrate that CoPA can also benefit existing learning-based PCQA models.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{5379} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2024}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{Contrastive Pre-Training with Multi-View Fusion for No-Reference PCQA}  % **** Enter the paper title here

% \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
% \noindent\textcolor{blue}{Response to NMvd's Q1 and hfZd's Q2: using existing networks (Swin-T and ResNet) as encoders.} \textbf{Ans:} Our key contribution lies in the pre-training framework (CoPA). Ideally, CoPA can achieve the expected performance on any network. Therefore, instead of using a specific PCQA network, we adopt simple backbones as encoders and outperform all SOTA NR-PCQA methods. In addition, we used CoPA to pre-train two NR-PCQA methods and obviously improved their prediction accuracy (see Table 4), further demonstrating the effectiveness of our pre-training strategy.

% \noindent\textcolor{blue}{B25b Q1: Generation of positive samples using patch-mixing is debatable.} \textbf{Ans:} In CoPA, positive samples are not defined by identical quality scores due to inaccessibility during pre-training. Therefore, we consider two factors (content and distortion) that are closely related to quality to generate positive samples. Given two projected images A and B with the same content but different distortions, the merged image retains the content and incorporates distortions from A and B. Consequently, we treat A and B as positive samples. Meanwhile, given the substantial presence of blank backgrounds within projected images, patch mixing can better preserve the integrity of the content compared to the cropping method used in IQA contrastive pre-training.


% \noindent\textcolor{blue}{B25b Q2: Results of just using features obtained from CoPA.} \textbf{Ans:} We directly use max-pooling to integrate multi-view features and a linear regressor to regress the features from frozen encoder following Re-IQA, and perform CoPA+FT to show the effect of pre-training and fine-tuning:
% \begin{table}[h]\tiny
% \vspace{-0.7cm}
% \centering 
% \renewcommand\tabcolsep{2.5pt}
% \renewcommand\arraystretch{0.7}
% % \resizebox{\textwidth}{12mm}
% \tiny
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
%     \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{LS-PCQA} & \multicolumn{3}{c|}{SJTU-PCQA} & \multicolumn{3}{c}{WPC} \\ 
%          & SRCC      & PLCC        & RMSE   & SRCC      & PLCC        & RMSE     & SRCC      & PLCC          & RMSE  \\ \hline
%  \textbf{only CoPA} & {0.598}& {0.624} & {0.170}  & {0.840} & {0.870} &
%  {0.121} & {0.759} & {0.772} &  {0.151} \\
%  \textbf{CoPA+FT} & {0.606}& {0.629} & {0.164}  & {0.841} & {0.872} &
%  {0.099} & {0.778} & {0.782} &  {0.147} \\

% \bottomrule
% \end{tabular}
% \label{tab:1}
% \vspace{-0.5cm}
% \end{table}

% \noindent\textcolor{blue}{B25b Q3: Results with ranking loss.}\textbf{Ans:} Results on SJTU are 0.725(SRCC),0.756(PLCC).We will add this in Table 3.

% \noindent\textcolor{blue}{NMvd Q1: Unique attribute information of point clouds.} \textbf{Ans:} We utilize the characteristics of point clouds in two ways: \textbf{1)} Unlike natural images, point clouds in PCQA datasets are single humans or objects, and their projected images include substantial blank background elements. Therefore, instead of cropping images like IQA methods, we use patch-mixing to generate positive samples, which can better preserve the content integrity. \textbf{2)} To fully exploit the attribute information of the point clouds from different perspectives, we apply multiple rotations to the point clouds before projection to achieve data augmentation.

% \noindent\textcolor{blue}{NMvd Q2: About $\mathcal{L}_d$ and $\mathcal{L}_c$.} \textbf{Ans:} $\mathcal{L}_d$ and $\mathcal{L}_c$ both range from 0 to $\infty$, and $\mathcal{L}_d$ is usually 2-4 times greater than $\mathcal{L}_c$ in scale. Therefore, we empirically set $\lambda$ to 0.3 in Formula 4 to balance the scales of $\mathcal{L}_d$ and $\mathcal{L}_c$.

% \noindent\textcolor{blue}{NMvd Q3: Can the training strategies of various datasets be unified?} \textbf{Ans:} We unify the training strategies into 5-fold cross validation, and the train-test ratio for LS-PCQA is 4:1. The result on LS-PCQA is updated as follows:
% \begin{table}[h]\small
% \renewcommand\tabcolsep{3.3pt}
% 	\centering
%  \renewcommand\arraystretch{0.6}
%     % \vspace{-0.3cm}
%   \tiny
% 	\begin{tabular}{c|cccccc}
% 		\toprule  % 顶部线
% 		   & PQA-Net & IT-PCQA & GPA-Net & ResSCNN & MM-PCQA & Ours \\
% 	SRCC & 0.583 & 0.337 & 0.587 & \bf\textcolor{blue}{0.593} & 0.587 & \bf\textcolor{red}{0.614}\\
% 	PLCC & 0.590 & 0.348 & 0.606 & \bf\textcolor{blue}{0.625} & 0.603 &\bf\textcolor{red}{0.638} \\
% 	RMSE & 0.199 & 0.226 & 0.192 & \bf\textcolor{blue}{0.170} & 0.191 & \bf\textcolor{red}{0.160} \\
% 		\bottomrule  % 底部线
% 	\end{tabular}
% 	\label{tab:2}
%  \vspace{-0.7cm}
% \end{table}

% \noindent\textcolor{blue}{NMvd Q4: Result with only FT.} \textbf{Ans:} Please see Table 3 (index \circled{2}) of our paper, and we will move this to Table 1. 

% \noindent\textcolor{blue}{NMvd Q5: Result obtained by training on LS and testing on SJTU/WPC.} \textbf{Ans:} Please see Table 2 of our paper.

% \noindent\textcolor{blue}{NMvd Q6: Using ResSCNN and MM-PCQA for visualization.} \textbf{Ans:} We use PQA-Net and GPA-Net to show the superiority of CoPA over distortion type prediction, as we discussed in Sec.1 and Sec.4.3. According to the suggestion of the reviewer, we add the result of ResSCNN and MM-PCQA as follows (please zoom in):
% \begin{figure}[h]
% \vspace{-0.4cm}
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/tsne_rebuttal.png}
%     \vspace{-0.4cm}
% \end{figure}

% \noindent\textcolor{blue}{NMvd Q7: About Fig.1.} \textbf{Ans:} More details of CoPA will be added in Introduction to make Fig.1 more understandable.

% \noindent\textcolor{blue}{NMvd Q8: About the encoder and pre-training.} \textbf{Ans:} In CoPA, the encoder encodes patch mixed images and projected images and is pre-trained to learn quality-aware features, which can be used to extract features from projected images of each view. CoPA works well because we define the positive/negative samples based on two factors (content and distortion) that are closely related to perceptual quality. The encoder without pre-training can be directly used with suboptimal performance (see Table 3 index \circled{2}).

% \noindent\textcolor{blue}{NMvd Q9: How to understand positive/negative samples?} \textbf{Ans:} Positive/negative samples are defined based on point cloud content and distortion. For the anchor (patch-mixed image), the positive samples are the two images used to generate the anchor because they share the same content with the anchor and the distortions are correlated. Positive samples should be closer to the anchor in the feature space. Conversely, negative samples are images projected from different reference point clouds, or with different distortions from the positive samples.

% \noindent\textcolor{blue}{hfZd Q1: Details of multi-view fusion.} \textbf{Ans:} The multi-view images are simply spatially stitched into one composed image. The encoder $\mathcal{G}$ is pre-trained on ImageNet for image classification, which focuses on high-level semantic information and can be used as a common practice to extract semantic features.

% \noindent\textcolor{blue}{hfZd Q3: About content and distortion.} \textbf{Ans:}
% We take content and distortion into consideration by our carefully designed negative samples, which can be divided into content-wise and distortion-wise ones to make the network extract features related to content and distortion, respectively. 

% \noindent\textcolor{blue}{hfZd Q4: Ranking loss.} \textbf{Ans:} In a mini-batch, the distances between any two scores $q_i,q_j$ (and $\hat{q}_i, \hat{q}_j$) are calculated to compare the relative ranking order.
% $i$,$j$ represent the $i$-th and $j$-th samples in the mini-batch. 

% %%%%%%%%% REFERENCES
% % {
% %     \small
% %     \bibliographystyle{ieeenat_fullname}
% %     \bibliography{main}
% % }

% \end{document}

